SkipNode: On Alleviating Performance Degradation for Deep Graph Convolutional Networks

Graph Convolutional Networks (GCNs) suffer from performance degradation when models go deeper. However, earlier works only attributed the performance degeneration to over-smoothing. In this paper, we conduct theoretical and experimental analysis to explore the fundamental causes of performance degradation in deep GCNs: over-smoothing and gradient vanishing have a mutually reinforcing effect that causes the performance to deteriorate more quickly in deep GCNs. On the other hand, existing anti-over-smoothing methods all perform full convolutions up to the model depth. They could not well resist the exponential convergence of over-smoothing due to model depth increasing. In this work, we propose a simple yet effective plug-and-play module, Skipnode, to overcome the performance degradation of deep GCNs. It samples graph nodes in each convolutional layer to skip the convolution operation. In this way, both over-smoothing and gradient vanishing can be effectively suppressed since (1) not all nodes'features propagate through full layers and, (2) the gradient can be directly passed back through ``skipped'' nodes. We provide both theoretical analysis and empirical evaluation to demonstrate the efficacy of Skipnode and its superiority over SOTA baselines.

==> tables/large.tex <==
%\begin{table}[ht]
%    \centering
%    \caption{\centering{Node Classification Accuracy (\%) on A Large Graph, i.e., ogbn-arxiv. $L = n$ indicates a n-layer model.}} 
%    \begin{tabular}{c c | c c c c}
%         \toprule
%         Backbone & Strategy & L = 10 & L = 12 & L = 14 & L = 16 \\
%         \midrule
%         \multirow{4}{*}{GCN} & -
%         & 66.5 & 62.3 & 58.7 & 53.2\\
%
%         ~ & \dropedge
%          & 66.7 & 62.8 & 60.3 & 55.1 \\
%
%         ~ & \textbf{\skipnodeu}
%         & \textbf{67.3} & \textbf{65.6} & 62.0 & 56.3\\
%       
%         ~ & \textbf{\skipnodeb} & 67.0 & 65.4 & \textbf{62.1} & \textbf{58.5} \\
%         \bottomrule
%    \end{tabular}
%    \label{table:ogbn-arxiv-accuray} 
%\end{table} 


%\begin{table}[ht]
%    \centering
%    \caption{\centering{Node Classification Accuracy (\%) on A Large Graph, i.e., ogbn-arxiv. $L = n$ indicates a n-layer model.}} 
%    \begin{tabular}{c c | c c c c}
%         \toprule
%         Backbone & Strategy & L = 10 & L = 12 & L = 14 & L = 16 \\
%         \midrule
%         \multirow{4}{*}{GCN} & -
%         & 66.5 & 62.3 & 58.7 & 53.2\\
%
%         ~ & \dropedge
%          & 66.7 & 62.8 & 60.3 & 55.1 \\
%
%         ~ & \textbf{\skipnodeu}
%         & \textbf{67.3} & \textbf{65.6} & 62.0 & 56.3\\
%       
%         ~ & \textbf{\skipnodeb} & 67.0 & 65.4 & \textbf{62.1} & \textbf{58.5} \\
%         \bottomrule
%    \end{tabular}
%    \label{table:ogbn-arxiv-accuray} 
%\end{table} 

\begin{table}[ht]
    \centering
     \caption{Link Prediction Results of GCN on ogbl-ppa.}
     \begin{tabular}{c c | c c | c c c}
         \toprule
         Dataset & Metric & Backbone & Strategy & L = 4 & L = 6 & L = 8 \\
         \midrule
         \multirow{3}{*}{ogbn-arxiv} & \multirow{3}{*}{Accuracy} & \multirow{3}{*}{GraphSAGE} & - & ~ & ~ & ~\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & ~ & ~ & ~ \\
         ~ & ~ & ~ & \textbf{\skipnodeb} & ~ & ~ & ~ \\
         \midrule
         \multirow{9}{*}{ogbl-ppa} & \multirow{3}{*}{Hits@10} & \multirow{3}{*}{GCN} & - & 3.19 & 5.29 & 3.68\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & 3.11 & \textbf{5.86} & \textbf{7.25}\\
         ~ & ~ & ~ & \textbf{\skipnodeb} & \textbf{3.48} & 5.72 & 5.86\\
         
%         \midrule
         ~ & \multirow{3}{*}{Hits@50} & \multirow{3}{*}{GCN} & - & 11.92 & 13.61 & 12.83\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & 12.01 & \textbf{14.95} & 14.39\\
         ~ & ~ & ~ & \textbf{\skipnodeb} & \textbf{13.31} & 14.17 & \textbf{14.95}\\
         
%         \midrule
         ~ & \multirow{3}{*}{Hits@100} & \multirow{3}{*}{GCN} & - & 17.11 & 18.54 & 16.50\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & \textbf{17.57} & \textbf{18.92} & \textbf{19.08}\\
         ~ & ~ & ~ & \textbf{\skipnodeb} & 17.54 & 18.74 & 18.92\\
         
         \bottomrule
    \end{tabular}
    \label{tab:ogbl-ppa-accuracy}
\end{table}


\begin{table}[ht]
    \centering
     \caption{Link Prediction Results of GCN on ogbl-ppa.}
     \begin{tabular}{c c | c c | c c c}
         \toprule
         Dataset & Metric & Backbone & Strategy & L = 4 & L = 6 & L = 8 \\
         \midrule
         \multirow{3}{*}{ogbn-arxiv} & \multirow{3}{*}{Accuracy} & \multirow{3}{*}{GraphSAGE} & - & ~ & ~ & ~\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & ~ & ~ & ~ \\
         ~ & ~ & ~ & \textbf{\skipnodeb} & ~ & ~ & ~ \\
         \midrule
         \multirow{9}{*}{ogbl-ppa} & \multirow{3}{*}{Hits@10} & \multirow{3}{*}{GCN} & - & 3.19 & 5.29 & 3.68\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & 3.11 & \textbf{5.86} & \textbf{7.25}\\
         ~ & ~ & ~ & \textbf{\skipnodeb} & \textbf{3.48} & 5.72 & 5.86\\
         
%         \midrule
         ~ & \multirow{3}{*}{Hits@50} & \multirow{3}{*}{GCN} & - & 11.92 & 13.61 & 12.83\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & 12.01 & \textbf{14.95} & 14.39\\
         ~ & ~ & ~ & \textbf{\skipnodeb} & \textbf{13.31} & 14.17 & \textbf{14.95}\\
         
%         \midrule
         ~ & \multirow{3}{*}{Hits@100} & \multirow{3}{*}{GCN} & - & 17.11 & 18.54 & 16.50\\
         ~ & ~ & ~ & \textbf{\skipnodeu} & \textbf{17.57} & \textbf{18.92} & \textbf{19.08}\\
         ~ & ~ & ~ & \textbf{\skipnodeb} & 17.54 & 18.74 & 18.92\\
         
         \bottomrule
    \end{tabular}
    \label{tab:ogbl-ppa-accuracy}
\end{table}
